Trustworthy and Efficient LLMs Meet Databases

In the rapidly evolving AI era with large language models (LLMs) at the core, making LLMs more trustworthy and efficient, especially in output generation (inference), has gained significant attention. This is to reduce plausible but faulty LLM outputs (a.k.a hallucinations) and meet the highly increased inference demands. This tutorial explores such efforts and makes them transparent to the database community. Understanding these efforts is essential in harnessing LLMs in database tasks and adapting database techniques to LLMs. Furthermore, we delve into the synergy between LLMs and databases, highlighting new opportunities and challenges in their intersection. This tutorial aims to share with database researchers and practitioners essential concepts and strategies around LLMs, reduce the unfamiliarity of LLMs, and inspire joining in the intersection between LLMs and databases.

==> 02.background.tex <==
\section{Background}\label{sec:background}

%\kmkim{Explain in detail including KQV, O, ...}
%\kmkim{running size = number of running requests}
%\kmkim{batch size}

This section explains the processing of LLM requests and related work.

\subsection{Processing a Single LLM Request}\label{subsec:background:single}

%inference cycle
%- prefill - take input prompt from CPU, model from GPU, generate KV, store KV to GPU
%- decode - 
%- KV, KV cache
%- preempt, evict
%- refill 

%\kmkim{TODO: add figure about input, layer, KV cache}

The input text of an LLM request is called \emph{prompt}.
When a request is sent to an LLM inference system, the system processes its prompt tokens and generates a new token. This step is called \emph{prefill}, followed by \emph{decode} steps, taking the last generated token and generating a new token sequentially. The decode phase ends if the last token is the end-of-sequence token or the number of generated tokens reaches a predefined limit. %This limit can be specified by the system or users, where 
The model also has a predefined \emph{context size}, which we denote as $C$, the maximum number of tokens the model can process at each step.


Processing a step includes 1) embedding the input $c$ tokens ($c \geq 1$ for prefill, $c = 1$ for decode) into $c$ vectors, 2) sending the vectors to GPU, and 3) performing matrix multiplications between the input vectors and model weights, and other GPU operations such as \emph{attentions} \cite{attention}.
The output vectors are the same size as the input vectors.
Step 3) repeats as many times as the number of model layers. %taking the input vectors from the previous layer and generating vectors for the next layer.
The output of the final layer is passed to a sampling part that generates a new token for the next step.
%3) loading the model weights (matrices) from GPU memory,

Most LLMs are based on the Transformer architecture with attention mechanism \cite{attention} to better utilize long contexts. %The attention is a model-free operation independent to model weights.
For each vector of the $i$-th token $x_i$, key (K), query (Q), and value (V) vectors, denoted by $K_i$, $Q_i$, and $V_i$, are generated from matrix multiplications. The query $Q_i$ and the key of every previous token, $K_{j \leq i}$, are used to compute the {weight} $w_{i,j}$ between $x_i$ and $x_j$. The weighted sum of $V_{j \leq i}$ with these weights is the output of attention for $x_i$. %This output is then passed to other matrix multiplications in the same layer.
The time complexity for $x_i$ is $O(i)$, thus the total complexity increases quadratically ($O(1 + 2 + ...)$) for a sequence of tokens.
From that $K_j$ and $V_j$ are reused for subsequent tokens $\{x_{k > j}\}$, keys and values are computed once and cached in GPU memory to avoid recomputation.
This is called \emph{key-value (KV) caching} \cite{KVCache}, a de facto standard for an efficient LLM inference.


Note that prefill tokens have no previous tokens to read KV's from, whereas decode tokens have an increasing number of KV's to read as the output length increases. 
%(from now on, we use KV as a unit size of K and V per token).
This makes prefills and decodes typically \emph{compute-bound} and \emph{decode-bound} \cite{SARATHI}. 
%respectively, but the exact classification depends on the prompt size, batch size (number of requests), and GPU's computation and memory bandwidth capacities \cite{LLMViewer}. % LLM Viewer


\subsection{Processing Multiple LLM Requests}\label{subsec:background:multiple}


As database systems are not free from interference between different user requests, LLM inference systems consider interference and resource utilization under multiple requests. 
Here, the resource mainly refers to two: the model's context size $C$ and the maximum KV cache size $M$ in terms of the number of tokens. Typically, $M$ is set as $\frac{available\_GPU\_memory - model\_size}{KV\_size\_per\_token}$, where the available GPU memory is less than the total memory capacity, e.g., 90\% in \cite{vLLM}.
%$M$ is typically set as the GPU capacity - model size.
The total number of tokens to process per batch cannot exceed $C$, and the total number of KV's stored in the cache cannot exceed $M$.


To enhance inference efficiency, systems have developed techniques similar to traditional database systems and operating systems.
The two standard techniques are \emph{continuous batching} \cite{Orca} and \emph{paged attention} \cite{vLLM}, each of which focuses on the computational and memory utilization of GPUs.
%Systems prior to continuous batching naively batched the requests and waited for every request in each batch to finish, before scheduling another batch of requests. This obviously led to inefficient \emph{bubbles}, underutilization of GPU computation, due to waiting for the longest request in a batch. Continuous batching instead schedules new requests after each prefill or decode step, if any of the previous request finishes and resource becomes available.
Continuous batching is to schedule new requests whenever there are enough resources, instead of waiting for all requests in the current batch to finish.
Paged attention increases memory utilization by managing KV cache in pages, instead of preallocating a large slot for every request (typically set to $C$). 
%This reduces 
%allowing flexible maintenance of KV per request.
%decoupling memory allocation
%Before the paged attention, the each request was given a predefined budget (e.g., the context size of the model) to store its all KV's, which limited the request throughput as only few requests can be scheduled, and a substantial part of memory was fragmented and underutilized \cite{vLLM}.


\emph{Hybrid batching} and \emph{chunked prefill} \cite{SARATHI, SARATHI_SERVE} are yet another approaches to schedule LLM requests. 
The hybrid batching is to simply batch prefill- and decode-phase requests together. %, to piggyback relatively short decodes to longer prefills (typically prefills take longer time to execute than decodes due to large prompts).
However, as prefills can be orders of magnitude heavier than decodes due to large prompts \cite{SARATHI}, decodes wait for longer prefills in the same batch to finish. 
To reduce this increased delay, chunked prefill allows partial processing of prompts per prefill. 
Here, $P$ ($\leq C$) is specified as the maximum number of prefill tokens per batch. Note that the generation of a new token occurs only when all the prompt tokens are processed.


%\SARATHI \cite{SARATHI, SARATHI_SERVE} partitions long prompts into smaller chunks and forms hybrid batches of prefill and decode requests, in order to reduce the large latency gap between prefill and decode, thus reducing computational wastes (bubbles). %chunked prefill, hybrid batching \\


%Finally, we define the \emph{batch size} as 


%\kmkim{TODO: add figure about request x time}


We define two notations of \emph{batch size} and \emph{running size} as follows. The former is the number of requests scheduled in a batch. The latter indicates the number of running requests holding KV's in the cache, which is larger than the batch size as some requests may hold KV's (thus running) but not being processed in certain batches.


Finally, as multiple requests store their KV's under the same budget of $M$, overloading the requests with too large running sizes can lead to \emph{preemption} of other running requests, releasing their KV's from the cache. We call these \emph{evictions} in the paper.
Once a request is evicted, all its generated tokens that have been sent back to the system are added to the prompt, and the request is rescheduled later \cite{vLLM}. We call this the \emph{refill} phase to differentiate with prefills.


%These approaches can be categorized based on their optimization focus:
%\kmkim{TODO: add citation, say that scalability is the real problem, easier to claim}
%\kmkim{While increasing the scalability of LLM inference remains as a challenge, due to the limited memory capacity of GPUs to sustain large KV cache.}
%Existing methods are constrained by the memory capacity of GPUs, which limits throughput as each token’s KV cache consumes substantial memory \cite{}.
%Offloading KV caches to CPU memory and streaming back to GPU is hampered by low PCIe bandwidth, preventing real-time access to offloaded data unless compromising accuracy \cite{InfiniGen}. 
%\kmkim{Compression-based methods also have a trade-off of accuracy or online decompression overhead \cite{}.}



%\kmkim{TODO: add figure about request x time - prefill/decode/hybrid/chunked/evict/refill, M, batch size, running size, }


%\kmkim{Figure \ref{fig:intro:sarathi} shows a simple example running \Vidur with \SARATHI scheduler. As previously mentioned, requests are scheduled until the KV cache reaches the limit and then preempted. Our approach can identify the wasted time for preempting and rescheduling the requests.}



%\kmkim{Model and pipeline parallelism play a crucial role in scaling inference, with pipeline parallelism partitioning model layers to different GPUs and model parallelism splitting a layer to multiple GPUs.}



\iffalse
\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{figure/sarathi_schedule.png}
\caption{An example of running \SARATHI scheduler implemented in \Vidur for 128 requests each of which takes 1024 input tokens and outputs 512 tokens. Yellow and gray cells represent requests in prefill and decode phases. Red and green lines show the occupancy ratio of KV cache and the number of preempted requests per iteration.}\label{fig:intro:sarathi}
\end{figure}
\fi


% can put it to the back
\subsection{Related Work}\label{subsec:related}

%\subsection{LLM Inference Systems}\label{subsec:related:system}

\iffalse
%NVLink: https://medium.com/gpgpu/multi-gpu-programming-6768eeb42e2c
\begin{figure}[h!]
\centering
\includegraphics[width=0.85\columnwidth]{figure/workflow.pdf}
\caption{Workflow of LLM inference with model parallelism.}\label{fig:workflow}
\end{figure}
\fi

%This section explains related work in LLM inference systems. %other than the ones explained previously.
% Taxonomy
%Explain previous approaches. Provide a taxonomy.
%Every method uses KV cache.
\noindent \underline{\textbf{LLM Inference System.}}
\Orca \cite{Orca} proposes continuous batching, \vLLM \cite{vLLM} proposes paged attention, and \SARATHI \cite{SARATHI, SARATHI_SERVE} proposes hybrid batching and chunked prefill.
%, enable requests to be scheduled without waiting for all previous requests to finish. % iteration-level scheduling, selective batching \\
%\vLLM \cite{vLLM} introduces paged attention, adapting paging and virtual memory in operating systems to tackle fragmentations in managing KV cache.
%\SARATHI \cite{SARATHI, SARATHI_SERVE} partitions long prompts into smaller chunks and forms hybrid batches of prefill and decode requests, in order to reduce the large latency gap between prefill and decode, thus reducing computational wastes (bubbles). %chunked prefill, hybrid batching \\
Instead of hybrid batching, \DistServe \cite{DistServe} and \Dejavu \cite{Dejavu} disaggregate prefill and decode phases by using different GPUs, sending the KV cache from the prefill to decode-handling GPU. % disaggregating prefill and decode \\
%- \Dejavu \cite{Dejavu}: disaggregating prefill and decode, streaming KV cache from prefill to decode layer-wise \\
\vTensor \cite{vTensor} decouples the KV cache allocation and attention computation in \vLLM, removing the page address translation overhead. This enables a similar performance with native attention techniques (e.g., FlashAttention \cite{FlashAttention}) when deployed to \vTensor.
% and allowing users to easily deploy new attention techniques.
%and preallocated KV cache in \vLLM, and proposes to dynamically allocate KV cache and decouple page translation and GPU kernels. % memory allocation and attention computation, reducing overheads and achieving similar performance with native FlashAttention, easier to implement new kernels \\
\InfiniGen \cite{InfiniGen} offloads the KV's to CPU for a larger KV cache using CPU memory and reloads the KV cache from CPU layer-wise. To minimize the data transfer overhead, it streams only the KV of the most important tokens and approximates the full attention result.
%and fetch the KV of important tokens to reduce data transfer overhead and further attentions \\
\NanoFlow \cite{NanoFlow} proposes a finer-grained batching than the continuous batching, where each batch of requests is further partitioned into nano-batches.
\InstInfer \cite{InstInfer} uses flash drives to offload KV's and even attention computations.
%compute attentions.
We hope that our findings and methodologies can improve the performance of existing systems and the development cycle of new systems.
%This paper focuses on cost modeling of inferences%
%on the analysis  scheduling part of inference systems and inference time predictions.
%and generalizing our approach to model more complex systems 
%We expect that our approach in the paper can help developing a 

%for modeling more complex batching and storage hierarchies with multiple GPUs, CPUs, and flash drives, 

%\subsection{Attention}\label{subsec:related:attention}

\noindent \underline{\textbf{LLM Inference Simulation.}}
\Vidur \cite{Vidur} offers the execution times of GPU operators of various models (e.g., Llama-2-7B \cite{Llama2}) on recent GPUs, including A40, A100, and H100. It implements two representative schedulers of \vLLM and \SARATHI, and offers accurate predictions on execution times.
%it provides measured GPU times for different model and hardware configurations, which are accurate (up to 9\% relative error to the true performance) and precise (times are measured layer-by-layer).
However, its focus is on simulation and search, not on a comprehensive analysis nor a methodology for designing a better scheduler.
%While one can run schedulers and predict the request response times, 
On the other hand, \LLMViewer \cite{LLMViewer} uses theoretical hardware bounds (GPU FLOPS and memory bandwidth) to analyze the performance of a single batch on different hardware configurations, without considering scheduling.
While our work is based on the results of \Vidur, it is straightforward to exploit the hardware bounds in \cite{LLMViewer}, which is left as a future work.


\noindent \underline{\textbf{Output Size Prediction.}}
Some studies have tried to estimate or rank the output sizes of requests for the better scheduling \cite{OPrediction, OPrediction2, ORank}.
In contrast, our work focuses on assessing the feasibility of such studies, raising a more fundamental question of how large is room for improvement by utilizing the output sizes at all. %can actually improve performance.
Our findings in subsequent sections are also valid when requests have the same output size, one of which sheds lights on input sizes (Section \ref{subsec:analysis:evictions_always_bad}).


\noindent \underline{\textbf{Efficient Attention and Decoding Techniques.}}
Although there have been extensive studies on efficient attention and decoding techniques, such as FlashAttention \cite{FlashAttention}, sliding window attention \cite{SlidingWindowAttention}, and speculative decoding \cite{SpeculativeDecoding}, these are orthogonal to our focus on scheduling (but FlashAttention is by default enabled in \Vidur and \vLLM).



==> 04.bio.tex <==
\section{Biography}\label{sec:bio}

\textbf{Kyoungmin Kim} is a Post Doctoral Fellow in the School of Computer Sciences at EPFL in Switzerland.
His recent research interest covers the 1) intersection of LLMs and databases and 2) intersection of theory and practice for efficient OLAP processing, which is also related to the trustworthiness and efficiency of LLMs.
For the first time, he proposed formulating optimal LLM inference schedules as a constraint satisfaction problem and showed non-trivial findings. %and suggested to use cost models for LLM inference scheduling
He received his Ph.D. in Department of Convergence IT Engineering at POSTECH in August 2023. %, with dissertation entitled ``Boosting Cardinality Estimation for Graph/Relational Databases using Sampling, Synopsis, and Deep Learning.''
%His work broadly covered graph algorithms, streaming systems, worst-case optimal joins, cardinality estimation, GPU-based query processing, and machine learning, with
He is the author of 7 SIGMOD (1 Demo), 1 VLDB, and 1 PODS paper, which was the first PODS paper from Korea.
He has served as a PC member of VLDB 2024, ICDE 2025, and BTW Demo 2025.



\noindent\textbf{Anastasia Ailamaki} is a Professor of Computer Sciences at EPFL and the Director of the Data-Intensive Applications and Systems (DIAS) lab. She is also the co-founder of RAW Labs SA, a Swiss company developing real-time analytics infrastructures for heterogeneous big data. Formerly, she was an associate professor of computer science at Carnegie Mellon School of Computer Science. 
She is the recipient of ten Best Paper and Best Demo awards and the author of over 200 peer-reviewed articles published in such journals as the Conference on Innovative Data Systems Research, VLDB, SIGMOD, ACM Transactions on Database Systems.
She received numerous awards, including the ACM SIGMOD Edgar F. Codd Innovations Award, the IEEE TCDE Impact Award, and recognition as both an ACM and IEEE Fellow.
She was also Vice Chair of SIGMOD in 2019.


%In 2013 she received an ERC Consolidator Award for the ViDa: Transforming raw data into information through virtualization project. She is a Fellow of the IEEE and ACM, a member of Academia Europaea, and the Vice Chair of the Special Interest Group of Management of Data (SIGMOD) within the Association for Computing Machinery. She is a member of the Expert Network of the World Economic Forum and CRA-W mentor. In 2019, she received ACM SIGMOD Edgar F. Codd Innovations Award.
%She is the author of over 200 peer-reviewed articles published in such journals as the Conference on Innovative Data Systems Research, VLDB, SIGMOD, ACM Transactions on Database Systems.

==> 07.opportunity.tex <==
\section{Challenges and Opportunities}\label{sec:opportunity}

%\noindent \textbf{Note: Opportunities}

% Dimensions we can improve (do we consider LoRA??)
% Similar to Proteus
%The opportunities left. What could be changed? Show the trend of bandwidth and memory capacity over past few decades. Explain in various complementary dimensions.

%- [Hardware] New memory hierarchy, HW, and new data transfer paths for KV cache maintenance \\
%- [Data] (Regarding model and KV cache as data to manage, where activations can be ignored, taking 5\% according to \cite{}) New model architecture like SSMs to reduce the size of KV, new attentions like sliding attention, KV cache compression \\
%- [Workload] New adaptive scheduler considering memory hierarchy, dynamic workloads, and requests' output lengths, work sharing between requests with input-output relationship, gpt-o1 (strawberry) for powerful reasoning and heavier inference \\

%\noindent \textbf{Note: Research Questions}

%- What's the best configuration satisfying the SLO and minimizing the cost (renting GPUs)? \\
%- What's the bottleneck in HW and what if we use better HW? \\
%- What's the new options we could take in such cases? Streaming KV cache? \\
%- How far can we decrease KV size and increase inference performance? \\
%- Can we compress KV cache and perform attentions on the compressed form without decompressing overhead? \\
%- Other than the layerwise KV cache streaming, can we stream KV cache tokenwise inside per-layer attentions? \\
%- What's the optimal scheduler we could invent and how's it better compared to current ones? \\
%- How does it vary for different SLOs? Given SLOs, is there a scheduler that satisfies SLOs under current HW or should we add more devices? \\
%- What if we adaptively adjust the chunk size? \\
%- What if we selectively maintain KV cache for a subset of requests or steps? \\
%- What if we have a sequence of LLM requests where an output becomes a new input? Can we overlap some computation? \\
%- So, from the above new approaches, what would be the final savings? \\




%\noindent \textbf{Note: Plans}
 
%- Design a unified model with data transfer paths, considering HW, for all current methods (which determines the constants, limits, and variables in CSP) // \kmkim{Single GPU -> Single node -> Multi node} \\
%- Design a CSP for the optimal scheduling problem with knowledge of output sizes and solve it (workload based on existing ones, like ShareGPT) \kmkim{Single GPU -> Single node -> Multi node} \\
%- Set various objectives and constraints combination for different SLOs and schedulers \\
%- Analyze the profile-based cost model of \Vidur on varying batch, input, and output sizes, and check if this approaches the HW bottleneck or theoretical cost model based on HW specs (using FLOPS, bandwidth) \\
%- Propose to dynamically adjust the chunk size and P:D in \SARATHI by modifying the constraints in the CSP \kmkim{so far, best chunk size is around 512, depends on batch size, input length} \\
%- Propose how to predict output size, such as asking LLMs "how long will your answer be" in order to approach the optimal scheduler \\
%- Propose adaptive scheduling for dynamic workloads \\
%- Propose work sharing for requests with input-output relationship. Propose judiciously using variables instead of generating of the same text over and over again. For example, when I ask to generate something, this can be an input to another question. When I ask LLM to generate some code, it generates, but the next time I ask to fix only a part, it generates from the beginning! \\
%- Propose attention on compressed KV and check the accuracy loss \\
%- Measure the savings from using SSMs (Mamba, Jamba, Smol LM) \\




\subsection{Hardware}\label{subsec:hardware}

\noindent \textbf{KV cache offloading}

While offloading the generated KV to CPUs, other GPUs, and other nodes is often studied in the literature \cite{Dejavu, DistServe, CacheGen, NanoFlow}, they mostly assume that the offloaded KV is used much later. \cite{NanoFlow} says that, even for an extremely high throughput of generating tens of thousands of tokens per second, a bandwidth of less than 10GB/s is enough to offload the generated KV. However, to use the offloaded KV in the decode attentions, we need to read all of the KVs generated for the request (not just the one token generated in the previous batch), possibly with 100-1000x higher speed than the generation.
An effective way to stream KV from CPU to GPU is to load them layer-wise \cite{InfiniGen}, so loading the KV for the next layer can be overlapped with the computation of the current layer. Still, the overhead cannot be hidden completely as the bandwidth of PCI between CPU and GPU is low. 


Cerebras inference using SRAM only


\subsection{Data}\label{subsec:data}

\noindent \textbf{SSM}

As state space models (SSMs), do not use attentions unlike Transformers, they do not maintain KV but a constant-size state independent to the number of tokens processed. Therefore, SSMs' decode throughput is less bounded by the GPU memory. 
While state-of-the-art models are still built upon Transformers, SSMs are evolving with better performance, thus are suitable models for increasing the throughput with a trade-off of accuracy or used as proxy models for speculative decoding with Transformer-based models.


\noindent \textbf{Data compression} 




\subsection{Workload}\label{subsec:workload}


\noindent \textbf{Model selection}

Choose the right model for each task, even code synthesis for simple tasks that LLM overkills.


\noindent \textbf{Avoiding repeated generation}

Not generating the same thing again, for example in code generation, users often want only a specific part to be fixed. In such cases, when given a modification request, instead of generating the next output from the scratch, feed the previous output as a speculative decoding and observe when the tokens diverge. 

Automatically generate variables for certain chunks in input and output. For a code generation example, when asked "fix this part as follows," we could determine what "this" and focus on generating that part, while the remaining parts are not generated again but simply extracted from the previous chat. Here, we have an internal variable for the remaining parts.


\noindent \textbf{Prefix caching and bulk semantic processing}

\kmkim{prefix caching = start request with $m > 0$ (prefix matching and scheduling is done in CPU)}

While prefix (KV) caching for future requests \cite{SGLang} have been proposed, under high contention with limited GPU memory, KVs for prefixes should be stored outside GPUs and loaded right before running the future request with the same prefix. However, caching prefixes without knowing the workload distribution is risky, that requests could be dissimilar. It is unlikely to know when similar request will arrive, for which the waiting time wastes the resources. 

In contrast, what if there is a meta task that is known to ask similar requests to complete the task? \cite{LOTUS} proposes \emph{bulk semantic processing} with LLMs over both structured and unstructured data, with new operators called \emph{semantic} operators. For example, applying the same NL-based selection filter "is this relevant to X" for every row in a table using LLMs. We could also join and aggregate tables based on semantics. Here, if the same operator is applied to every row, we can share the prefix without an effort. The output size is also shorter and more controllable as the output will be boolean or new attribute for tables (e.g., just True or False for semantic filters). Therefore, the batches given to the inference scheduler will probably consists of prefills, and the advantages of maintaining KV cache could be small for individual items or rows, or rather incur unnecessary overheads due to address translation \cite{vTensor}.


\noindent \textbf{Mixed relational and semantic processing}

Add Viktor's work

New optimization opportunities

- Lazy materialization: we do not need to materialize the LLM output until it is accessed in parent operators, considering that it can be discarded due to relational filters and other operators.

- LLM pull-up: as LLM token generation is the most time-consuming operation, it is necessary to pull up LLM operators and push down lightweight relational operators.

- Overlapping CPU- and GPU-friendly operators: not only considering GPU kernel times for LLM query processing, need to consider CPU time for relational operators and how to overlap them. %Furthermore, GPU-based relational engines \cite{} 

- Higher priority for lower-level operators in the pipeline?

- Output of an operator becomes an input for the next operator, just like passing input and output tokens to the next iteration in GPT-o1. 


\noindent \textbf{Heavy reasoning and inference}

- Now we have Strawberry or GPT-o1.


